Inapproximability of a Pair of Forms Defining a Partial Boolean Function

We consider the problem of jointly minimizing forms of two Boolean functions $f, g \colon \{0,1\}^J \to \{0,1\}$ such that $f + g \leq 1$ and so as to separate disjoint sets $A \cup B \subseteq \{0,1\}^J$ such that $f(A) = \{1\}$ and $g(B) = \{1\}$. We hypothesize that this problem is easier to solve or approximate than the well-understood problem of minimizing the form of one Boolean function $h: \{0,1\}^J \to \{0,1\}$ such that $h(A) = \{1\}$ and $h(B) = \{0\}$. For a large class of forms, including binary decision trees and ordered binary decision diagrams, we refute this hypothesis. For disjunctive normal forms, we show that the problem is at least as hard as MIN-SET-COVER. For all these forms, we establish that no $o(\ln (|A| + |B| -1))$-approximation algorithm exists unless P$=$NP.

==> section-upper-bound.tex <==
Next, we construct a polynomial-time $\frac{1}{2}|J||A\cup B|$-approximation algorithm for \textsc{min-length-dnf}, which, for any Boolean labeled data $D=(J, X, A, B)$, outputs DNFs $(\theta, \theta')$ with $f_\theta^{-1}(1) = A$ and $f_{\theta'}^{-1}(1) = B$. 
%
Therefor, we approximate \textsc{min-length-dnf} by solving two instances of \textsc{min-set-cover} over the prime implicants 
\cite{Crama2011}
of the sets of truth points $A$ and false points $B$, respectively.
Finally, we show that our analysis of the approximation algorithm is essentially tight, by constructing an example which matches the approximation ratio.

\begin{definition}[\cite{Lukas1999}]
	For 
	any finite, non-empty set $J$, 
	the set $X = \{0,1\}^J$,
	the family $f \colon \Theta \to \{0,1\}^X$ of DNFs, and
	any non-empty set $A \subseteq X$, 
	the instance of \textsc{min-length-dnf-total} w.r.t. $(J, X, A)$ has the form
	\begin{align}
		\min_{\theta\in \Theta} \quad & R_l(\theta) & \\
		\textnormal{subj.~to} \quad & \forall x \in A\colon \quad f_{\theta}(x) = 1 & \textnormal{(exactness)}\\
		&\forall x\in X \setminus A\colon\quad f_{\theta}(x) = 0 & \textnormal{(exactness)}
	\end{align}
\end{definition}

It is well known and discussed comprehensively by \cite{Crama2011} that \textsc{min-length-dnf-total} can be polynomially reduced to \textsc{min-set-cover} by stating it as a covering problem over the prime implicants of the set $A$.
Via this reduction, \textsc{min-length-dnf-total} can be approximated such that, for any instance $(J, X, A)$, the approximate solution $\theta$ has the properties $\vert \theta\vert \leq \vert A\vert$ and $R_l(\theta) \leq \vert J \vert \vert A\vert$.

%\begin{lemma}
%	\textsc{min-length-dnf-total} is reducible to \textsc{min-set-cover}.
%\end{lemma}
%\begin{proof}
%	% The 'well-known' reduction using prime implicants.
%\end{proof}

%\begin{corollary}
%	\label{cor:algorithm-exact-dnf-minimization}
%	There is a greedy polynomial-time 
%	%$\ln \vert S\vert$-approximate 
%	approximation algorithm for \textsc{min-length-dnf-total}, which, for any labeled Boolean data $D$, returns a solution $\theta$ to the instance of \textsc{min-length-dnf-total} w.r.t. $D$ with $\vert \theta\vert \leq \vert S\vert$ and $R_l(\theta) \leq n \vert S\vert$.
%\end{corollary}

\begin{lemma}
	\label{lemma:simplealgorithm}
	For 
	any Boolean labeled data $(J, X, A, B) = D$, 
	the tuples $D_1 = (J, X, A)$ and $D_0 = (J, X, B)$,
	and the approximation algorithm $\mathcal{A}$ for \textsc{min-length-dnf-total}, 
	the algorithm $\mathcal{A}'$ such that 
	\begin{equation}
		\mathcal{A}'(D) = \left(\mathcal{A}(D_1), \mathcal{A}(D_0)\right)
	\end{equation}
	is a polynomial-time $\frac{1}{2}\vert J \vert\vert A \cup B\vert$-approximate algorithm for the instance of \textsc{min-length-dnf} w.r.t. $D$.
\end{lemma}

\begin{proof}
	Firstly, the algorithm $\mathcal{A}'$ outputs feasible solutions $\mathcal{A}'(D) = (\theta, \theta')$ in polynomial time, by construction. 
	%
	Secondly, for the optimal solution $(\hat{\theta}, \hat{\theta}')$ to the instance of \textsc{min-length-dnf} w.r.t. $D$:
	\begin{align}
		\frac{R_l(\theta)+R_l(\theta')}{R_l(\hat\theta)+R_l(\hat{\theta}')} &\leq \frac{R_l(\theta) + R_l(\theta')}{2} && \textnormal{($A, B\neq \emptyset$)} \\
		& \leq \frac{\vert J \vert}{2} \left(\vert A \vert + \vert B \vert \right) && \textnormal{(Prop. of $\mathcal{A}$)} \\
		& = \frac{\vert J \vert}{2} \vert A\cup B \vert && \textnormal{($A\cap B = \emptyset$)}
	\end{align}
\end{proof}
%
%\begin{lemma}
%	For any Boolean labeled data $D=(J, S, X, Y, x, y)$ with $S \neq \emptyset$ and
%	the optimal solution $(\hat{\theta}, \hat{\theta}')$ to the instance of \textsc{min-length-dnf} w.r.t. $D$,
%	the algorithm $\mathcal{A}'$ from Lemma~\ref{lemma:simplealgorithm} returns a feasible solution $\mathcal{A}'(D)=(\theta, \theta')$ such that 
%	\begin{equation}
%		\frac{R_l(\theta)+R_l(\theta')}{R_l(\hat\theta)+R_l(\hat{\theta}')} \leq n \vert S\vert\enspace.
%	\end{equation}
%\end{lemma}
%\begin{proof}
%	Firstly, it holds $S\neq \emptyset$ and therefore 
%	\begin{equation}
%		R_l(\hat{\theta})+R_l(\hat{\theta}') \geq 1\enspace.
%	\end{equation}
%	Secondly, by Corollary~\ref{cor:algorithm-exact-dnf-minimization},  the solutions $\theta$ and $\theta'$ returned by $\mathcal{A}$ are such that
%	\begin{align}
%		R_l(\theta) + R_l(\theta') \leq n \vert S\vert\enspace.
%	\end{align}
%	Therefore, it holds 
%	\begin{equation}
%		\frac{R_l(\theta)+R_l(\theta')}{R_l(\hat\theta)+R_l(\hat{\theta}')} \leq n \vert S\vert\enspace.
%	\end{equation}
%\end{proof}
%\begin{corollary}
%	The algorithm $\mathcal{A}'$ of Lemma~\ref{lemma:simplealgorithm} is a polynomial-time $n\vert S\vert$-approximate algorithm.
%\end{corollary}

Next, we show that the analysis of the approximation algorithm is essentially tight, by constructing an example which matches the approximation ratio.

\begin{lemma}
	For 
	any finite, non-empty set $J$,
	the set $X = \{0,1\}^J$, 
	the $x^i\in X$ such that 
	\begin{align}
		\forall i, j \in J \colon \quad x^i_j = \begin{cases}
			1 & \textnormal{if } i = j \\
			0 & \textnormal{otherwise}
		\end{cases}
		\enspace ,
	\end{align}
	any $k\in J$,
	the set $A = \{x^i \;|\; \ i\in J\setminus \{k\}\}$ and the set $B = \{x^k\}$,  
	the algorithm $\mathcal{A}'$ outputs a solution $(\theta, \theta')$ to the instance of \textsc{min-length-dnf} w.r.t.~$(J, X, A, B)$ with the approximation ratio $\frac{1}{2}\vert J \vert \vert A \cup B\vert$.
\end{lemma}

\begin{proof}
%	Let $D = (J, S, X, Y, x, y)$ be such that $S = y^{-1}(1)$ and $\vert S \vert = \vert J \vert$. Consider any bijection $s'\colon J \to S$, and $x\colon S \to X$ such that 
%	\begin{equation}
%		\forall i \in J\;\forall j\in J\colon x_{s'_i}(j) = \llbracket i = j\rrbracket\enspace.
%	\end{equation}
	For the instance of \textsc{min-length-dnf-total} w.r.t.~$D_1 = (J, X, A)$, the algorithm $\mathcal{A}$ outputs the DNF 
	\begin{align}
		\theta = \{(\{i\}, J \setminus \{i\}) \;\vert\; i\in J\setminus \{k\}\}
	\end{align}
	as this is the only feasible solution.
	
	For the instance of \textsc{min-length-dnf-total} w.r.t.~$D_0 = (J, X, B)$, 
	the algorithm $\mathcal{A}$ outputs the DNF
	\begin{align}
		\theta' = \{(\{k\}, J \setminus \{k\})\}
	\end{align} 
	as this is the only feasible solution. 
	
	Therefore, the total length of the DNFs output by $\mathcal{A}'$ is 
	\begin{equation}
		R_l(\theta) + R_l(\theta') = \vert J \vert \vert A\cup B\vert
		\enspace .
	\end{equation}
	The optimal solution to the instance of \textsc{min-length-dnf} w.r.t. $D$ 
	is $(\hat{\theta}, \hat{\theta}')$ such that 
	\begin{align}
		\hat{\theta} = \{(\emptyset, \{k\})\}\\
		\hat{\theta}' = \{(\{k\}, \emptyset)\}
	\end{align} 
	with length $R_l(\hat{\theta}) + R_l(\hat{\theta}') = 2$. Therefore, the approximation ratio is 
	\begin{equation}
		\frac{R_l(\mathcal{A}(D_1)) + R_l(\mathcal{A}(D_0))}{R_l(\hat{\theta})+R_l(\hat{\theta}')} = \frac{1}{2}\vert J \vert \vert A\cup B\vert 
		\enspace.
	\end{equation}
\end{proof}
% Since the observations $A\cup B$ lie in a subcube of dimension $n' \leq \vert A\cup B\vert$, we can w.l.o.g. assume, that $\vert A\cup B\vert \geq \vert J \vert$. Therefore, the approximation ratio and the tightness example can be replaced by a ratio of $\vert A\cup B\vert^2$.




















